Mixed flow ionospheric aerodynamics

The increasingly congested near earth environment requires accurate orbital modelling to prevent collision events that threaten access to space infrastructure. Ionospheric aerodynamics are the largest non-conservative source of orbital perturbations. Work done by Brown et al provided a prediction method for drag forces on charged bodies in low earth orbit based on applying approximations of single species flows to representative plasma simulations. Recent work on mixed species plasma sheaths motivates investigation of this assumption. Mixed species plasma flows over charged bodies with representative LEO conditions were simulated, focusing on orbital motion limited O$^+$ dominated flows, and sheath limited H$^+$ dominated flows. The significance of small concentrations of different ion species was analysed in terms of aerodynamic effects on the body. Introduction of small concentrations of H$^+$ into a flow dominated by O$^+$ molecules showed significant disruptions to the wake structure, coupled with an increase in drag coefficient for a satellite in that flow. Introducing heavier O$^+$ molecules into a sheath dominated H$^+$ flow found little disruption to the wake structure. A multi-species drag model was proposed, building on work in Brown et al. This model was found to qualitatively describe changes in wake structure, but consistently over predicted drag coefficients. This finding suggests that the influence of mixed species flows on ionospheric aerodynamics involves significant contributions from inter-species interactions not described adequately by considering the separate species as either separate flows, or one flow with adjusted parameters.

==> BackgroundTemplates/binding.tex <==
\chapter{Binding}\label{C:bin}

The Library states:
\begin{itemize}
\item Thesis must be fully bound and cased in cloth or buckram in optional colour. (I think they mean you can pick the colour!)
\item Author's surname and initials and (short) title lettered on spine. (The thesis's title, not the author's, presumably.)
\item Author's full name and full title lettered on front cover. (Again, the thesis's title, not the author's, presumably.)
\item Two copies of a PhD thesis and one copy of a Master's thesis must be deposited. A signed availability slip must accompany the thesis.
\item  The principal supervisor is responsible for the deposit.
\end{itemize}

==> BackgroundTemplates/thestyle.tex <==
\chapter{The front pages}\label{C:ex}

You can declare:
\begin{itemize}
\item an author using  \verb+\author{}+ -- your full name;
\item a title using \verb+\title{}+-- ALL IN CAPITALS IN THE EXAMPLE, but we use \verb#\Large# and \verb#\bf#, so normal case will do;
\item a subject using \verb+\subject{}+-- probably Computer Science, but you can pick anything you like;
\item an abstract using \verb+\abstract{}+-- this should be fewer then 500 words for a PhD. The handbook states ``A length of about 300 words is recommended.'' The \textsf{book} style does not have an \verb+abstract+ environment defined, so this is a bit of a hack.
\end{itemize}

You can also specify what degree you are submitting the thesis for by using:
\begin{itemize}
\item  \verb+\phd+, which produces ``\ldots in fulfilment of \ldots Doctor of Philosophy''
\item  \verb+\mscthesisonly+, which produces ``\ldots in fulfilment of \ldots Master of Science''
\item  \verb+\mscwithhonours+, which produces ``\ldots in partial fulfilment of \ldots Master of Science with Honours''
\item  \verb+\mscbothparts+, which produces ``\ldots in partial fulfilment of \ldots Master of Science''
\item  \verb+\otherdegree{DEGREE OR DIPLOMA NAME}+, which produces ``\ldots in fulfilment of \ldots DEGREE OR DIPLOMA NAME''
\end{itemize}

